Identifying Gene-Environment Interactions with A Least Relative Error Approach

For complex diseases, the interactions between genetic and environmental risk factors can have important implications beyond the main effects. Many of the existing interaction analyses conduct marginal analysis and cannot accommodate the joint effects of multiple main effects and interactions. In this study, we conduct joint analysis which can simultaneously accommodate a large number of effects. Significantly different from the existing studies, we adopt loss functions based on relative errors, which offer a useful alternative to the "classic" methods such as the least squares and least absolute deviation. Further to accommodate censoring in the response variable, we adopt a weighted approach. Penalization is used for identification and regularized estimation. Computationally, we develop an effective algorithm which combines the majorize-minimization and coordinate descent. Simulation shows that the proposed approach has satisfactory performance. We also analyze lung cancer prognosis data with gene expression measurements.

==> self-define-HL.tex <==

\def\brown{\color{brown}}
\def\blue{\color{blue}}
\def\green{\color{green}}
\def\red{\color{red}}
 

\def\tbrown{\textcolor{brown}}
\def\tred{\textcolor{red}}
\def\tcyan{\textcolor{cyan}}
\def\tblue{\textcolor{blue}}
 
\def\hlnote#1#2{{
    \bf \color{red} #1: \color{blue}  #2
        }}
\def\delete#1{\iffalse #1 \fi}

\def\hlcomment#1{\vskip 2mm\boxit{\vskip 2mm{\color{blue}\bf#1} {\color{green}\sf \hfill--HL\vskip 2mm}}\vskip 2mm}


 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        ITEM and equation environments                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\itemitem{\par\indent \hangindent2\parindent}
\newcommand{\labelitemv}{$\oslash$}%{$\clubsuit$}

 
\renewcommand{\labelitemi}{$\bullet$}  %{$\Diamond$}
\renewcommand{\labelitemii}{$\diamond$}%\circ$} %{$\spadesuit$}%{$\circ$}
\renewcommand{\labelitemiii}{$---$}%{$\diamond$}%{$\circ$}
\renewcommand{\labelitemiv}{$\ast$}%{$\clubsuit$}


%\newcommand{\mat}[3]{\mathop{\mathstrut #1}\limits_{\raise.5em\hbox{$\scriptstyle #2\times#3$}}}
%\newcommand{\usim}[1]{\mathop{\mathstrut #1}\limits_{\raise20em\hbox{$\sim$}}}
%\def\be{\begin{eqnarray}}
\def\bse{\begin{eqnarray*}}
%\def\ee{\end{eqnarray}}
\def\ese{\end{eqnarray*}}
\def\bee{\begin{enumerate}}
\def\eee{\end{enumerate}}
\def\bqe{\begin{eqnarray}}
\def\eqe{\end{eqnarray}}
\def\bed{\begin{description}}
\def\eed{\end{description}}
\def\bei{\begin{itemize}}
\def\eei{\end{itemize}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        Common mathematical macros                          %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\cumsum{\mbox{cumsum}}
\def\real{{\mathbb R}}
\def\sumin{\sum_{i=1}^n}
\def\sumjn{\sum_{j=1}^n}
\def\sumkn{\sum_{k=1}^n}
\def\sumkK{\sum_{k=1}^K}
\def\sumjd{\sum_{j=1}^d}
\def\sui{\sum_{i=1}^n}
\def \suj{\sum_{j=1}^n}
\def \suji{\sum_{j=1}^n\sum_{i=1}^n}
\def \suij{\sum_{i=1}^n\sum_{j=1}^n}
\def \ixti{I_{(X_i \le x, T_i\le t)}}
\def \ixtj{I_{(X_j \le x, T_j\le t)}}
\def\implies{\Longrightarrow}
\def\ifandonlyif{\Longleftrightarrow}
\def\infint{\int_{-\infty}^{\infty}}
\def\transpose{{\sf T}}

\def\smhalf{{\textstyle{1\over2}}}
\def\third{{\textstyle{1\over3}}}
\def\twothirds{{\textstyle{2\over3}}}
\def\threeeighths{{\textstyle{3\over8}}}
\def\threequarters{{\textstyle{3\over4}}}
\def\quarter{{\textstyle{1\over4}}}
\def\approxdist{\stackrel{{\tiny \mbox{approx.}}}{\sim}}
\def\eqdist{\stackrel{{\tiny \mbox{dist.}}}{=}}
\def\simiid{\stackrel{{\tiny \mbox{i.i.d.}}}{\sim}}
\def\simind{\stackrel{{\tiny \mbox{ind.}}}{\sim}}
\def\lla{\longleftarrow}
\def\lra{\longrightarrow}
\def\Lla{\Longleftarrow}
\def\Lra{\Longrightarrow}
\def\Ra{\Rightarrow}
\def\llra{\longleftrightarrow}
\def\Llra{\Longleftrightarrow}
\def\TOL{\TagsOnLeft}
\def\TOR{\TagsOnRight}

\def\convdist{\stackrel{\cal D}{\lra}}
\def\convprob{\stackrel{\cal P}{\lra}}

\def\dotovrka{\buildrel . \over {\kappa}}
\def\dotovrM{\buildrel . \over M}
\def\dotovrm{\buildrel . \over m}
\def\dotovrV{\buildrel . \over V}
\def\dotovrK{\buildrel . \over K}
\def\dotovrsg{\buildrel . \over {\sigma}}
\def\dotovrVK{\buildrel . \over {\VK}}
\def\dotovrX{\buildrel . \over X}
\def\dotovrVX{\buildrel . \over {\VX}}
\def\dotorVM{\buildrel . \over {\VM}}
\def\dotorVV{\buildrel . \over {\VV}}
\def\pmb#1{\setbox0=\hbox{#1}%
    \kern-.025em\copy0\kern-\wd0
    \kern.05em\copy0\kern-\wd0
    \kern-.025em\raise.0433em\box0 }
\def\pmbh#1#2{\setbox0=\hbox{#1}%
    \setbox1=\hbox{#2}%
    \kern-.025em\copy0\kern-\wd0
    \kern.05em\copy1\kern-\wd0
    \kern-.025em\raise.0433em\box0 }

%\def\overset{\stackrel{\rm def}{=}}
\def\overset{\stackrel{\Delta}{=}}
\def\R{\mbox{I}\!\mbox{R}}
\def\binom#1#2{{#1\choose #2}}
\def\frac#1#2{{#1\over#2}}
\def\dfrac#1#2{{\displaystyle{#1\over#2}}}
\def\dsum{\displaystyle{\sum}}
\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern6pt
   \vbox{\kern6pt#1\kern6pt}\kern6pt\vrule}\hrule}}
\def\refhg{\hangindent=20pt\hangafter=1}
\def\refmark{\par\vskip 2mm\noindent\refhg}
\def\non{\nonumber}

\newcommand{\boxtab}[1]{\smallskip
\begin{center}\fbox{ \rule[-.5cm]{0cm}{1.2cm}{\tt Put Table #1 here}}
\end{center}\smallskip}
\newcommand{\boxfig}[1]{\smallskip
\begin{center}\fbox{ \rule[-.5cm]{0cm}{1.2cm} {\tt Put Figure #1 here}}
\end{center}\smallskip}

\def\vhrule{\hrule\vskip 1mm}
\def\bhrule{\vskip 1mm\hrule\vskip 1mm}
\def\blackbox{\hfill\rule{.15in}{.15in}}

\def\listing#1{\vskip 4mm\begin{verbatim}\input#1 \vskip 4mm}
\def\thick#1{\hbox{\rlap{$#1$}\kern0.25pt\rlap{$#1$}\kern0.25pt$#1$}}
\def\ol{\overline}
\def\ob{\overbrace}
\def\ul{\underline}
\def\ub{\underbrace}
\def\wt{\widetilde}
\def\wh{\widehat}
\def\n{\noindent}
\def\ve{\varepsilon}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              Common text abbreviations                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\etal{{\rm et al.}}
\def\bias{\mbox{bias}}
\def\var{\mbox{var}}
\def\cov{\mbox{cov}}
\def\ols{{\mbox{\rm\tiny OLS}}}
\def\gls{{\mbox{\rm\tiny GLS}}}
\def\wls{{\mbox{\rm\tiny WLS}}}
\def\ml{{\mbox{\rm\tiny ML}}}
\def\rml{{\mbox{\rm\tiny RML}}}
\def\mle{{\mbox{\rm\tiny MLE}}}
\def\reml{{\mbox{\rm\tiny REML}}}
\def\lme{{\mbox{\rm\tiny LME}}}
\def\nlme{{\mbox{\rm\tiny NLME}}}

\def\tr{{\mbox{\rm tr}}}
\def\T{{\mbox{\rm\tiny T}}}
\def\diag{{\mbox{\rm diag}}}
\def\chf{\hfill}   % for canceling conveniently in further%%%%%%%%%
\def\iid{\mbox{i.i.d.}}
\def\diff{d\,}
\def\Diff{{\sf D}}
\def\Hess{{\sf H}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              Roman Letters                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Bf Roman Letters	 %
%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bfa{{\bf a}}  \def\bfA{{\bf A}}
\def\bfb{{\bf b}}  \def\bfB{{\bf B}}
\def\bfc{{\bf c}}  \def\bfC{{\bf C}}
\def\bfd{{\bf d}}  \def\bfD{{\bf D}}
\def\bfe{{\bf e}}  \def\bfE{{\bf E}}
\def\bff{{\bf f}}  \def\bfF{{\bf F}}
\def\bfg{{\bf g}}  \def\bfG{{\bf G}}
\def\bfh{{\bf h}}  \def\bfH{{\bf H}}
\def\bfi{{\bf i}}  \def\bfI{{\bf I}}
\def\bfj{{\bf j}}  \def\bfJ{{\bf J}}
\def\bfk{{\bf k}}  \def\bfK{{\bf K}}
\def\bfl{{\bf l}}  \def\bfL{{\bf L}}
\def\bfm{{\bf m}}  \def\bfM{{\bf M}}
\def\bfn{{\bf n}}  \def\bfN{{\bf N}}
\def\bfo{{\bf o}}  \def\bfO{{\bf O}}
\def\bfp{{\bf p}}  \def\bfP{{\bf P}}
\def\bfq{{\bf q}}  \def\bfQ{{\bf Q}}
\def\bfr{{\bf r}}  \def\bfR{{\bf R}}
\def\bfs{{\bf s}}  \def\bfS{{\bf S}}
\def\bft{{\bf t}}  \def\bfT{{\bf T}}
\def\bfu{{\bf u}}  \def\bfU{{\bf U}}
\def\bfv{{\bf v}}  \def\bfV{{\bf V}}
\def\bfw{{\bf w}}  \def\bfW{{\bf W}}
\def\bfx{{\bf x}}  \def\bfX{{\bf X}}
\def\bfy{{\bf y}}  \def\bfY{{\bf Y}}
\def\bfz{{\bf z}}  \def\bfZ{{\bf Z}}
\def\bfzero{{\bf 0}}
\def\bfone{{\bf 1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Boldmath Roman Letters       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bolda{{\mbox{\boldmath $a$}}}   \def\boldA{{\mbox{\boldmath $A$}}}
\def\boldb{{\mbox{\boldmath $b$}}}   \def\boldB{{\mbox{\boldmath $B$}}}
\def\boldc{{\mbox{\boldmath $c$}}}   \def\boldC{{\mbox{\boldmath $C$}}}
\def\boldd{{\mbox{\boldmath $d$}}}   \def\boldD{{\mbox{\boldmath $D$}}}
\def\bolde{{\mbox{\boldmath $e$}}}   \def\boldE{{\mbox{\boldmath $E$}}}
\def\boldf{{\mbox{\boldmath $f$}}}   \def\boldF{{\mbox{\boldmath $F$}}}
\def\boldg{{\mbox{\boldmath $g$}}}   \def\boldG{{\mbox{\boldmath $G$}}}
\def\boldh{{\mbox{\boldmath $h$}}}   \def\boldH{{\mbox{\boldmath $H$}}}
\def\boldi{{\mbox{\boldmath $i$}}}   \def\boldI{{\mbox{\boldmath $I$}}}
\def\boldj{{\mbox{\boldmath $j$}}}   \def\boldJ{{\mbox{\boldmath $J$}}}
\def\boldk{{\mbox{\boldmath $k$}}}   \def\boldK{{\mbox{\boldmath $K$}}}
\def\boldl{{\mbox{\boldmath $l$}}}   \def\boldL{{\mbox{\boldmath $L$}}}
\def\boldm{{\mbox{\boldmath $m$}}}   \def\boldM{{\mbox{\boldmath $M$}}}
\def\boldn{{\mbox{\boldmath $n$}}}   \def\boldN{{\mbox{\boldmath $N$}}}
\def\boldo{{\mbox{\boldmath $o$}}}   \def\boldO{{\mbox{\boldmath $O$}}}
\def\boldp{{\mbox{\boldmath $p$}}}   \def\boldP{{\mbox{\boldmath $P$}}}
\def\boldq{{\mbox{\boldmath $q$}}}   \def\boldQ{{\mbox{\boldmath $Q$}}}
\def\boldr{{\mbox{\boldmath $r$}}}   \def\boldR{{\mbox{\boldmath $R$}}}
\def\bolds{{\mbox{\boldmath $s$}}}   \def\boldS{{\mbox{\boldmath $S$}}}
\def\boldt{{\mbox{\boldmath $t$}}}   \def\boldT{{\mbox{\boldmath $T$}}}
\def\boldu{{\mbox{\boldmath $u$}}}   \def\boldU{{\mbox{\boldmath $U$}}}
\def\boldv{{\mbox{\boldmath $v$}}}   \def\boldV{{\mbox{\boldmath $V$}}}
\def\boldw{{\mbox{\boldmath $w$}}}   \def\boldW{{\mbox{\boldmath $W$}}}
\def\boldx{{\mbox{\boldmath $x$}}}   \def\boldX{{\mbox{\boldmath $X$}}}
\def\boldy{{\mbox{\boldmath $y$}}}   \def\boldY{{\mbox{\boldmath $Y$}}}
\def\boldz{{\mbox{\boldmath $z$}}}   \def\boldZ{{\mbox{\boldmath $Z$}}}
%%%%%%%%%%%%%%%%%%%%%%%%
%  pmb Roman Letters   %
%%%%%%%%%%%%%%%%%%%%%%%%
\def\pmba{{\pmb a}} \def\pmbA{{\pmb A}}
\def\pmbb{{\pmb b}} \def\pmbB{{\pmb B}}
\def\pmbc{{\pmb c}} \def\pmbC{{\pmb C}}
\def\pmbd{{\pmb d}} \def\pmbD{{\pmb D}}
\def\pmbe{{\pmb e}} \def\pmbE{{\pmb E}}
\def\pmbf{{\pmb f}} \def\pmbF{{\pmb F}}
\def\pmbg{{\pmb g}} \def\pmbG{{\pmb G}}
\def\pmbh{{\pmb h}} \def\pmbH{{\pmb H}}
\def\pmbi{{\pmb i}} \def\pmbI{{\pmb I}}
\def\pmbj{{\pmb j}} \def\pmbJ{{\pmb J}}
\def\pmbk{{\pmb k}} \def\pmbK{{\pmb K}}
\def\pmbl{{\pmb l}} \def\pmbL{{\pmb L}}
\def\pmbm{{\pmb m}} \def\pmbM{{\pmb M}}
\def\pmbn{{\pmb n}} \def\pmbN{{\pmb N}}
\def\pmbo{{\pmb o}} \def\pmbO{{\pmb O}}
\def\pmbp{{\pmb p}} \def\pmbP{{\pmb P}}
\def\pmbq{{\pmb q}} \def\pmbQ{{\pmb Q}}
\def\pmbr{{\pmb r}} \def\pmbR{{\pmb R}}
\def\pmbs{{\pmb s}} \def\pmbS{{\pmb S}}
\def\pmbt{{\pmb t}} \def\pmbT{{\pmb T}}
\def\pmbu{{\pmb u}} \def\pmbU{{\pmb U}}
\def\pmbv{{\pmb v}} \def\pmbV{{\pmb V}}
\def\pmbw{{\pmb w}} \def\pmbW{{\pmb W}}
\def\pmbx{{\pmb x}} \def\pmbX{{\pmb X}}
\def\pmby{{\pmb y}} \def\pmbY{{\pmb Y}}
\def\pmbz{{\pmb z}} \def\pmbZ{{\pmb Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Calligraphic Roman Letters %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\calA{{\cal A}}
\def\calB{{\cal B}}
\def\calC{{\cal C}}
\def\calD{{\cal D}}
\def\calE{{\cal E}}
\def\calF{{\cal F}}
\def\calG{{\cal G}}
\def\calH{{\cal H}}
\def\calI{{\cal I}}
\def\calJ{{\cal J}}
\def\calK{{\cal K}}
\def\calL{{\cal L}}
\def\calM{{\cal M}}
\def\calN{{\cal N}}
\def\calO{{\cal O}}
\def\calP{{\cal P}}
\def\calQ{{\cal Q}}
\def\calR{{\cal R}}
\def\calS{{\cal S}}
\def\calT{{\cal T}}
\def\calU{{\cal U}}
\def\calV{{\cal V}}
\def\calW{{\cal W}}
\def\calX{{\cal X}}
\def\calY{{\cal Y}}
\def\calZ{{\cal Z}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Small thick Roman Letters	 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\sthicka{{\thick{\scriptstyle{a}}}}   \def\sthickA{{\thick{\scriptstyle{A}}}}
\def\sthickb{{\thick{\scriptstyle{b}}}}   \def\sthickB{{\thick{\scriptstyle{B}}}}
\def\sthickc{{\thick{\scriptstyle{c}}}}   \def\sthickC{{\thick{\scriptstyle{C}}}}
\def\sthickd{{\thick{\scriptstyle{d}}}}   \def\sthickD{{\thick{\scriptstyle{D}}}}
\def\sthicke{{\thick{\scriptstyle{e}}}}   \def\sthickE{{\thick{\scriptstyle{E}}}}
\def\sthickf{{\thick{\scriptstyle{f}}}}   \def\sthickF{{\thick{\scriptstyle{F}}}}
\def\sthickg{{\thick{\scriptstyle{g}}}}   \def\sthickG{{\thick{\scriptstyle{G}}}}
\def\sthickh{{\thick{\scriptstyle{h}}}}   \def\sthickH{{\thick{\scriptstyle{H}}}}
\def\sthicki{{\thick{\scriptstyle{i}}}}   \def\sthickI{{\thick{\scriptstyle{I}}}}
\def\sthickj{{\thick{\scriptstyle{j}}}}   \def\sthickJ{{\thick{\scriptstyle{J}}}}
\def\sthickk{{\thick{\scriptstyle{k}}}}   \def\sthickK{{\thick{\scriptstyle{K}}}}
\def\sthickl{{\thick{\scriptstyle{l}}}}   \def\sthickL{{\thick{\scriptstyle{L}}}}
\def\sthickm{{\thick{\scriptstyle{m}}}}   \def\sthickM{{\thick{\scriptstyle{M}}}}
\def\sthickn{{\thick{\scriptstyle{n}}}}   \def\sthickN{{\thick{\scriptstyle{N}}}}
\def\sthicko{{\thick{\scriptstyle{o}}}}   \def\sthickO{{\thick{\scriptstyle{O}}}}
\def\sthickp{{\thick{\scriptstyle{p}}}}   \def\sthickP{{\thick{\scriptstyle{P}}}}
\def\sthickq{{\thick{\scriptstyle{q}}}}   \def\sthickQ{{\thick{\scriptstyle{Q}}}}
\def\sthickr{{\thick{\scriptstyle{r}}}}   \def\sthickR{{\thick{\scriptstyle{R}}}}
\def\sthicks{{\thick{\scriptstyle{s}}}}   \def\sthickS{{\thick{\scriptstyle{S}}}}
\def\sthickt{{\thick{\scriptstyle{t}}}}   \def\sthickT{{\thick{\scriptstyle{T}}}}
\def\sthicku{{\thick{\scriptstyle{u}}}}   \def\sthickU{{\thick{\scriptstyle{U}}}}
\def\sthickv{{\thick{\scriptstyle{v}}}}   \def\sthickV{{\thick{\scriptstyle{V}}}}
\def\sthickw{{\thick{\scriptstyle{w}}}}   \def\sthickW{{\thick{\scriptstyle{W}}}}
\def\sthickx{{\thick{\scriptstyle{x}}}}   \def\sthickX{{\thick{\scriptstyle{X}}}}
\def\sthicky{{\thick{\scriptstyle{y}}}}   \def\sthickY{{\thick{\scriptstyle{Y}}}}
\def\sthickz{{\thick{\scriptstyle{z}}}}   \def\sthickZ{{\thick{\scriptstyle{Z}}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Arrowed Roman Letters  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%These are AMS constructs for horizontal arrows
% need include tacilatex.sty
%\input c:/tex-lib-hua/sty-need/tcilatex.sty
%\input tcilatex.sty
\def\aarrow{\underrightarrow{a}}  \def\Aarrow{\underrightarrow{A}}
\def\barrow{\underrightarrow{b}}  \def\Barrow{\underrightarrow{B}}
\def\carrow{\underrightarrow{c}}  \def\Carrow{\underrightarrow{C}}
\def\darrow{\underrightarrow{d}}  \def\Darrow{\underrightarrow{D}}
\def\earrow{\underrightarrow{e}}  \def\Earrow{\underrightarrow{E}}
\def\farrow{\underrightarrow{f}}  \def\Farrow{\underrightarrow{F}}
\def\garrow{\underrightarrow{g}}  \def\Garrow{\underrightarrow{G}}
\def\harrow{\underrightarrow{h}}  \def\Harrow{\underrightarrow{H}}
\def\iarrow{\underrightarrow{i}}  \def\Iarrow{\underrightarrow{I}}
\def\jarrow{\underrightarrow{j}}  \def\Jarrow{\underrightarrow{J}}
\def\karrow{\underrightarrow{k}}  \def\Karrow{\underrightarrow{K}}
\def\larrow{\underrightarrow{l}}  \def\Larrow{\underrightarrow{L}}
\def\marrow{\underrightarrow{m}}  \def\Marrow{\underrightarrow{M}}
\def\narrow{\underrightarrow{n}}  \def\Narrow{\underrightarrow{N}}
\def\oarrow{\underrightarrow{o}}  \def\Oarrow{\underrightarrow{O}}
\def\parrow{\underrightarrow{p}}  \def\Parrow{\underrightarrow{P}}
\def\qarrow{\underrightarrow{q}}  \def\Qarrow{\underrightarrow{Q}}
\def\rarrow{\underrightarrow{r}}  \def\Rarrow{\underrightarrow{R}}
\def\sarrow{\underrightarrow{s}}  \def\Sarrow{\underrightarrow{S}}
\def\tarrow{\underrightarrow{t}}  \def\Tarrow{\underrightarrow{T}}
\def\uarrow{\underrightarrow{u}}  \def\Uarrow{\underrightarrow{U}}
\def\varrow{\underrightarrow{v}}  \def\Varrow{\underrightarrow{V}}
\def\warrow{\underrightarrow{w}}  \def\Warrow{\underrightarrow{W}}
\def\xarrow{\underrightarrow{x}}  \def\Xarrow{\underrightarrow{X}}
\def\yarrow{\underrightarrow{y}}  \def\Yarrow{\underrightarrow{Y}}
\def\zarrow{\underrightarrow{z}}  \def\Zarrow{\underrightarrow{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \wt\ul\bf Roman letters	            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\wtuba{\wt{\ul{\bf a}}} \def\wtubA{\wt{\ul{\bf A}}}
\def\wtubb{\wt{\ul{\bf b}}} \def\wtubB{\wt{\ul{\bf B}}}
\def\wtubc{\wt{\ul{\bf c}}} \def\wtubC{\wt{\ul{\bf C}}}
\def\wtubd{\wt{\ul{\bf d}}} \def\wtubD{\wt{\ul{\bf D}}}
\def\wtube{\wt{\ul{\bf e}}} \def\wtubE{\wt{\ul{\bf E}}}
\def\wtubf{\wt{\ul{\bf f}}} \def\wtubF{\wt{\ul{\bf F}}}
\def\wtubg{\wt{\ul{\bf g}}} \def\wtubG{\wt{\ul{\bf G}}}
\def\wtubh{\wt{\ul{\bf h}}} \def\wtubH{\wt{\ul{\bf H}}}
\def\wtubi{\wt{\ul{\bf i}}} \def\wtubI{\wt{\ul{\bf I}}}
\def\wtubj{\wt{\ul{\bf j}}} \def\wtubJ{\wt{\ul{\bf J}}}
\def\wtubk{\wt{\ul{\bf k}}} \def\wtubK{\wt{\ul{\bf K}}}
\def\wtubl{\wt{\ul{\bf l}}} \def\wtubL{\wt{\ul{\bf L}}}
\def\wtubm{\wt{\ul{\bf m}}} \def\wtubM{\wt{\ul{\bf M}}}
\def\wtubn{\wt{\ul{\bf n}}} \def\wtubN{\wt{\ul{\bf N}}}
\def\wtubo{\wt{\ul{\bf o}}} \def\wtubO{\wt{\ul{\bf O}}}
\def\wtubp{\wt{\ul{\bf p}}} \def\wtubP{\wt{\ul{\bf P}}}
\def\wtubq{\wt{\ul{\bf q}}} \def\wtubQ{\wt{\ul{\bf Q}}}
\def\wtubr{\wt{\ul{\bf r}}} \def\wtubR{\wt{\ul{\bf R}}}
\def\wtubs{\wt{\ul{\bf s}}} \def\wtubS{\wt{\ul{\bf S}}}
\def\wtubt{\wt{\ul{\bf t}}} \def\wtubT{\wt{\ul{\bf T}}}
\def\wtubu{\wt{\ul{\bf u}}} \def\wtubU{\wt{\ul{\bf U}}}
\def\wtubv{\wt{\ul{\bf v}}} \def\wtubV{\wt{\ul{\bf V}}}
\def\wtubw{\wt{\ul{\bf w}}} \def\wtubW{\wt{\ul{\bf W}}}
\def\wtubx{\wt{\ul{\bf x}}} \def\wtubX{\wt{\ul{\bf X}}}
\def\wtuby{\wt{\ul{\bf y}}} \def\wtubY{\wt{\ul{\bf Y}}}
\def\wtubz{\wt{\ul{\bf z}}} \def\wtubZ{\wt{\ul{\bf Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  \wh\ul\bf Roman letters	      %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\whuba{\wh{\ul{\bf a}}} \def\whubA{\wh{\ul{\bf A}}}
\def\whubb{\wh{\ul{\bf b}}} \def\whubB{\wh{\ul{\bf B}}}
\def\whubc{\wh{\ul{\bf c}}} \def\whubC{\wh{\ul{\bf C}}}
\def\whubd{\wh{\ul{\bf d}}} \def\whubD{\wh{\ul{\bf D}}}
\def\whube{\wh{\ul{\bf e}}} \def\whubE{\wh{\ul{\bf E}}}
\def\whubf{\wh{\ul{\bf f}}} \def\whubF{\wh{\ul{\bf F}}}
\def\whubg{\wh{\ul{\bf g}}} \def\whubG{\wh{\ul{\bf G}}}
\def\whubh{\wh{\ul{\bf h}}} \def\whubH{\wh{\ul{\bf H}}}
\def\whubi{\wh{\ul{\bf i}}} \def\whubI{\wh{\ul{\bf I}}}
\def\whubj{\wh{\ul{\bf j}}} \def\whubJ{\wh{\ul{\bf J}}}
\def\whubk{\wh{\ul{\bf k}}} \def\whubK{\wh{\ul{\bf K}}}
\def\whubl{\wh{\ul{\bf l}}} \def\whubL{\wh{\ul{\bf L}}}
\def\whubm{\wh{\ul{\bf m}}} \def\whubM{\wh{\ul{\bf M}}}
\def\whubn{\wh{\ul{\bf n}}} \def\whubN{\wh{\ul{\bf N}}}
\def\whubo{\wh{\ul{\bf o}}} \def\whubO{\wh{\ul{\bf O}}}
\def\whubp{\wh{\ul{\bf p}}} \def\whubP{\wh{\ul{\bf P}}}
\def\whubq{\wh{\ul{\bf q}}} \def\whubQ{\wh{\ul{\bf Q}}}
\def\whubr{\wh{\ul{\bf r}}} \def\whubR{\wh{\ul{\bf R}}}
\def\whubs{\wh{\ul{\bf s}}} \def\whubS{\wh{\ul{\bf S}}}
\def\whubt{\wh{\ul{\bf t}}} \def\whubT{\wh{\ul{\bf T}}}
\def\whubu{\wh{\ul{\bf u}}} \def\whubU{\wh{\ul{\bf U}}}
\def\whubv{\wh{\ul{\bf v}}} \def\whubV{\wh{\ul{\bf V}}}
\def\whubw{\wh{\ul{\bf w}}} \def\whubW{\wh{\ul{\bf W}}}
\def\whubx{\wh{\ul{\bf x}}} \def\whubX{\wh{\ul{\bf X}}}
\def\whuby{\wh{\ul{\bf y}}} \def\whubY{\wh{\ul{\bf Y}}}
\def\whubz{\wh{\ul{\bf z}}} \def\whubZ{\wh{\ul{\bf Z}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Bf Roman Letters   9/5/2010 %
%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mbfa{\mathbf{a}}  \def\mbfA{\mathbf{A}}
\def\mbfb{\mathbf{b}}  \def\mbfB{\mathbf{B}}
\def\mbfc{\mathbf{c}}  \def\mbfC{\mathbf{C}}
\def\mbfd{\mathbf{d}}  \def\mbfD{\mathbf{D}}
\def\mbfe{\mathbf{e}}  \def\mbfE{\mathbf{E}}
\def\mbff{\mathbf{f}}  \def\mbfF{\mathbf{F}}
\def\mbfg{\mathbf{g}}  \def\mbfG{\mathbf{G}}
\def\mbfh{\mathbf{h}}  \def\mbfH{\mathbf{H}}
\def\mbfi{\mathbf{i}}  \def\mbfI{\mathbf{I}}
\def\mbfj{\mathbf{j}}  \def\mbfJ{\mathbf{J}}
\def\mbfk{\mathbf{k}}  \def\mbfK{\mathbf{K}}
\def\mbfl{\mathbf{l}}  \def\mbfL{\mathbf{L}}
\def\mbfm{\mathbf{m}}  \def\mbfM{\mathbf{M}}
\def\mbfn{\mathbf{n}}  \def\mbfN{\mathbf{N}}
\def\mbfo{\mathbf{o}}  \def\mbfO{\mathbf{O}}
\def\mbfone{\mathbf{1}}
\def\mbfp{\mathbf{p}}  \def\mbfP{\mathbf{P}}
\def\mbfq{\mathbf{q}}  \def\mbfQ{\mathbf{Q}}
\def\mbfr{\mathbf{r}}  \def\mbfR{\mathbf{R}}
\def\mbfs{\mathbf{s}}  \def\mbfS{\mathbf{S}}
\def\mbft{\mathbf{t}}  \def\mbfT{\mathbf{T}}
\def\mbfu{\mathbf{u}}  \def\mbfU{\mathbf{U}}
\def\mbfv{\mathbf{v}}  \def\mbfV{\mathbf{V}}
\def\mbfw{\mathbf{w}}  \def\mbfW{\mathbf{W}}
\def\mbfx{\mathbf{x}}  \def\mbfX{\mathbf{X}}
\def\mbfy{\mathbf{y}}  \def\mbfY{\mathbf{Y}}
\def\mbfz{\mathbf{z}}  \def\mbfZ{\mathbf{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                   Greek                                    %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Bf math Greek Letters   9/4/2010 %
%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\mbfalpha{\mathbf{\alpha}}   \def\mbfAlpha{\mathbf{\Alpha}}
\def\mbfbeta{\mathbf{\beta}}     \def\mbfBeta{\mathbf{\beta}}
\def\mbfdelta{\mathbf{\delta}}   \def\mbfDelta{\mathbf{\Delta}}
\def\mbfeta{\mathbf{\eta}}       \def\mbfEta{\mathbf{\Eta}}
\def\mbfgamma{\mathbf{\gamma}}   \def\mbfGamma{\mathbf{\Gamma}}
\def\mbflambda{\mathbf{\lambda}} \def\mbfLambda{\mathbf{\Lambda}}
\def\mbfmu{\mathbf{\mu}}         \def\mbfMu{\mathbf{\Mu}}
\def\mbfnu{\mathbf{\nu}}         \def\mbfNu{\mathbf{\Nu}}
\def\mbfomega{\mathbf{\omega}}   \def\mbfOmega{\mathbf{\Omega}}
\def\mbfpi{\mathbf{\pi}}         \def\mbfPi{\mathbf{\Pi}}
\def\mbfphi{\mathbf{\phi}}	 \def\mbfPhi{\mathbf{\Phi}}
\def\mbfpsi{\mathbf{\psi}}       \def\mbfPsi{\mathbf{\Psi}}
\def\mbfsigma{\mathbf{\sigma}}   \def\mbfSigma{\mathbf{\Sigma}}
\def\mbftheta{\mathbf{\theta}}   \def\mbfTheta{\mathbf{\Theta}}
\def\mbfve{\mathbf{\ve}}         \def\mbfVe{\mathbf{\Epsilon}}
\def\mbfxi{\mathbf{\xi}}         \def\mbfXi{\mathbf{\Xi}}
\def\mbfzeta{\mathbf{\zeta}}     \def\mbfZeta{\mathbf{\Zeta}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Bold Greek Letters	 %
%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\boldalpha{{\mbox{\boldmath $\alpha$}}}   \def\boldAlpha{{\mbox{\boldmath $\Alpha$}}}
\def\boldbeta{{\mbox{\boldmath $\beta$}}}     \def\boldBeta{{\mbox{\boldmath $\beta$}}}
\def\bolddelta{{\mbox{\boldmath $\delta$}}}   \def\boldDelta{{\mbox{\boldmath $\Delta$}}}
\def\boldeta{{\mbox{\boldmath $\eta$}}}       \def\boldEta{{\mbox{\boldmath $\Eta$}}}
\def\boldgamma{{\mbox{\boldmath $\gamma$}}}   \def\boldGamma{{\mbox{\boldmath $\Gamma$}}}
\def\boldlambda{{\mbox{\boldmath $\lambda$}}} \def\boldLambda{{\mbox{\boldmath $\Lambda$}}}
\def\boldmu{{\mbox{\boldmath $\mu$}}}         \def\boldMu{{\mbox{\boldmath $\Mu$}}}
\def\boldnu{{\mbox{\boldmath $\nu$}}}         \def\boldNu{{\mbox{\boldmath $\Nu$}}}
\def\boldomega{{\mbox{\boldmath $\omega$}}}   \def\boldOmega{{\mbox{\boldmath $\Omega$}}}
\def\boldpsi{{\mbox{\boldmath $\psi$}}}       \def\boldPsi{{\mbox{\boldmath $\Psi$}}}
\def\boldsigma{{\mbox{\boldmath $\sigma$}}}   \def\boldSigma{{\mbox{\boldmath $\Sigma$}}}
\def\boldpi{{\mbox{\boldmath $\pi$}}}         \def\boldPi{{\mbox{\boldmath $\Pi$}}}

\def\boldtheta{{\mbox{\boldmath $\theta$}}}   \def\boldTheta{{\mbox{\boldmath $\Theta$}}}
\def\boldve{{\mbox{\boldmath $\ve$}}}         \def\boldVe{{\mbox{\boldmath $\Epsilon$}}}
\def\boldxi{{\mbox{\boldmath $\xi$}}}         \def\boldXi{{\mbox{\boldmath $\Xi$}}}
\def\boldzeta{{\mbox{\boldmath $\zeta$}}}     \def\boldZeta{{\mbox{\boldmath $\Zeta$}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Thick Greek Letters	 %
%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\tgalpha{{\thick\alpha}}		  \def\tgAlpha{{\thick\Alpha}}
\def\tgbeta{{\thick\beta}}		  \def\tgBeta{{\thick\Beta}}
\def\tgchi{{\thick\chi}} 		  \def\tgChi{{\thick\Chi}}
\def\tgdelta{{\thick\delta}}		  \def\tgDelta{{\thick\Delta}}
\def\tggamma{{\thick\gamma}}		  \def\tgGamma{{\thick\Gamma}}
\def\tgepsilon{{\thick\epsilon}} 	  \def\tgEpsilon{{\thick\Epsilon}}
\def\tgve{{\thick\ve}}	              \def\tgZeta{{\thick\Zeta}}
\def\tgzeta{{\thick\zeta}}		  \def\tgEta{{\thick\Eta}}
\def\tgdeta{{\thick\eta}}		  \def\tgTheta{{\thick\Theta}}
\def\tgtheta{{\thick\theta}}		  \def\tgIota{{\thick\Iota}}
\def\tgiota{{\thick\iota}}		  \def\tgKappa{{\thick\Kappa}}
\def\tgkappa{{\thick\kappa}}		  \def\tgLambda{{\thick\Lambda}}
\def\tglambda{{\thick\lambda}}	  \def\tgMu{{\thick\Mu}}
\def\tgmu{{\thick\mu}}			  \def\tgNu{{\thick\Nu}}
\def\tgnu{{\thick\nu}}			  \def\tgXi{{\thick\Xi}}
\def\tgxi{{\thick\xi}}			  \def\tgOmicron{{\thick\Omicron}}
\def\tgomicron{{\thick\omicron}} 	  \def\tgPi{{\thick\Pi}}
\def\tgpi{{\thick\pi}}			  \def\tgRho{{\thick\Rho}}
\def\tgrho{{\thick\rho}} 		  \def\tgSigma{{\thick\Sigma}}
\def\tgsigma{{\thick\sigma}}		  \def\tgTau{{\thick\Tau}}
\def\tgtau{{\thick\tau}} 		  \def\tgUpsilon{{\thick\Upsilon}}
\def\tgupsilon{{\thick\upsilon}} 	  \def\tgPhi{{\thick\Phi}}
\def\tgphi{{\thick\phi}} 		  \def\tgPsi{{\thick\Psi}}
\def\tgpsi{{\thick\psi}} 		  \def\tgOmega{{\thick\Omega}}
\def\tgomega{{\thick\omega}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Small thick Greek Letters   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\stgalpha{{\thick{\scriptstyle{\alpha}}}}	     \def\stgAlpha{{\thick{\scriptstyle{\Alpha}}}}
\def\stgbeta{{\thick{\scriptstyle{\beta}}}}	     \def\stgBeta{{\thick{\scriptstyle{\Beta}}}}
\def\stggamma{{\thick{\scriptstyle{\gamma}}}}	     \def\stgGamma{{\thick{\scriptstyle{\Gamma}}}}
\def\stgdelta{{\thick{\scriptstyle{\delta}}}}	     \def\stgDelta{{\thick{\scriptstyle{\Delta}}}}
\def\stgepsilon{{\thick{\scriptstyle{\epsilon}}}}    \def\stgEpsilon{{\thick{\scriptstyle{\Epsilon}}}}
\def\stgve{{\thick{\scriptstyle{\ve}}}} 	           \def\stgZeta{{\thick{\scriptstyle{\Zeta}}}}
\def\stgzeta{{\thick{\scriptstyle{\zeta}}}}	     \def\stgEta{{\thick{\scriptstyle{\Eta}}}}
\def\stgdeta{{\thick{\scriptstyle{\eta}}}}	     \def\stgTheta{{\thick{\scriptstyle{\Theta}}}}
\def\stgtheta{{\thick{\scriptstyle{\theta}}}}	     \def\stgIota{{\thick{\scriptstyle{\Iota}}}}
\def\stgiota{{\thick{\scriptstyle{\iota}}}}	     \def\stgKappa{{\thick{\scriptstyle{\Kappa}}}}
\def\stgkappa{{\thick{\scriptstyle{\kappa}}}}	     \def\stgLambda{{\thick{\scriptstyle{\Lambda}}}}
\def\stglambda{{\thick{\scriptstyle{\lambda}}}}      \def\stgMu{{\thick{\scriptstyle{\Mu}}}}
\def\stgmu{{\thick{\scriptstyle{\mu}}}} 	           \def\stgNu{{\thick{\scriptstyle{\Nu}}}}
\def\stgnu{{\thick{\scriptstyle{\nu}}}} 	           \def\stgXi{{\thick{\scriptstyle{\Xi}}}}
\def\stgxi{{\thick{\scriptstyle{\xi}}}} 	           \def\stgOmicron{{\thick{\scriptstyle{\Omicron}}}}
\def\stgomicron{{\thick{\scriptstyle{\omicron}}}}    \def\stgPi{{\thick{\scriptstyle{\Pi}}}}
\def\stgpi{{\thick{\scriptstyle{\pi}}}} 	           \def\stgRho{{\thick{\scriptstyle{\Rho}}}}
\def\stgrho{{\thick{\scriptstyle{\rho}}}}	           \def\stgSigma{{\thick{\scriptstyle{\Sigma}}}}
\def\stgsigma{{\thick{\scriptstyle{\sigma}}}}	     \def\stgTau{{\thick{\scriptstyle{\Tau}}}}
\def\stgtau{{\thick{\scriptstyle{\tau}}}}	           \def\stgUpsilon{{\thick{\scriptstyle{\Upsilon}}}}
\def\stgupsilon{{\thick{\scriptstyle{\upsilon}}}}    \def\stgPhi{{\thick{\scriptstyle{\Phi}}}}
\def\stgphi{{\thick{\scriptstyle{\phi}}}}	           \def\stgChi{{\thick{\scriptstyle{\Chi}}}}
\def\stgchi{{\thick{\scriptstyle{\chi}}}}	           \def\stgPsi{{\thick{\scriptstyle{\Psi}}}}
\def\stgpsi{{\thick{\scriptstyle{\psi}}}}	           \def\stgOmega{{\thick{\scriptstyle{\Omega}}}}
\def\stgomega{{\thick{\scriptstyle{\omega}}}}

\renewcommand\today{\ifcase\month\or
   Jan\or Feb\or Mar\or Apr\or May\or
   Jun\or Jul\or Aug\or Sep\or Oct\or Nov\or
   Dec\fi
   \space\number\day, \number\year}

%%%%%%%%%%%%%%
%   THE END  %
%%%%%%%%%%%%%% 
